Contego: An Adaptive Framework for Integrating Security Tasks in Real-Time Systems

Embedded real-time systems (RTS) are pervasive. Many modern RTS are exposed to unknown security flaws, and threats to RTS are growing in both number and sophistication. However, until recently, cyber-security considerations were an afterthought in the design of such systems. Any security mechanisms integrated into RTS must (a) co-exist with the real- time tasks in the system and (b) operate without impacting the timing and safety constraints of the control logic. We introduce Contego, an approach to integrating security tasks into RTS without affecting temporal requirements. Contego is specifically designed for legacy systems, viz., the real-time control systems in which major alterations of the system parameters for constituent tasks is not always feasible. Contego combines the concept of opportunistic execution with hierarchical scheduling to maintain compatibility with legacy systems while still providing flexibility by allowing security tasks to operate in different modes. We also define a metric to measure the effectiveness of such integration. We evaluate Contego using synthetic workloads as well as with an implementation on a realistic embedded platform (an open- source ARM CPU running real-time Linux).

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

# LATEX = pdflatex 
LATEX = xelatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> Sections/background.tex <==
% \documentclass[../rt_server_main.tex]{subfiles}

% \begin{document}





\subsection{\remove[MH]{Overview of RTS}} \label{sec:background}

\remove[MH]{RTS are those that, apart from a requirement for functional correctness,
require that temporal properties be met as well. These temporal properties are often
presented in the form of \textit{deadlines}. The usefulness of results produced by the system
drops on the passage of a deadline. If the usefulness drops sharply then we refer to
the system as a  \textit{hard} real-time system (\eg avionics, nuclear power plants, 
anti-lock braking systems in automobiles, \etc) and if it drops in a more gradual manner 
then they are referred to as \textit{soft} real-time systems (\eg multimedia streaming, 
automated windshield wipers, \etc). %Figure \ref{fig:realtime_assumptions} lists 
As illustrated in Table \ref{tab:rts}, some
of the common properties/assumptions related to hard RTS include: periodic/sporadic execution of set of tasks, strict timing and safety requirements, bounded execution time, limited resources, \etc 

% \begin{inparaenum}[\em i\textnormal{)}]
% \item implemented as a system of periodic/sporadic tasks;
% \item stringent timing requirements;
% \item worst-case bounds are known for most loops;
% \item no dynamically loaded or self modified codes;
% \item recursion is either not used or statically bounded;
% \item memory and processing power is often limited.
% \end{inparaenum}



%\todo[inline]{Rod: bounds should be known for all loops, otherwise how do you compute WCET?}
%\hl{MH: fixed!}


RTS are often designed based on the Liu and Layland task model \cite{Liu_n_Layland1973}
that contains a set of tasks, $\Gamma$ where each task $\tau_i \in \Gamma$
has the parameters: $(C_i, T_i, D_i)$, where $C_i$ is
the worst-case execution time (WCET), $T_i$ is the period or minimum inter-arrival time, and $D_i$ is the deadline, with $D_i \leq T_i$.
Schedulability tests \cite{res_time_rts, bini2004schedulability} are used to determine
if all tasks in the system meet their respective deadlines. If they do, then the task set is deemed to be \textit{`schedulable'} and the system, \textit{safe}. }

\hl{MH: This table will be removed.}
\begin{table}[h t b] 
\centering
\caption{Properties of Majority RTS}
\label{tab:rts}
\begin{tabular}{|c p{6.5cm}|} \hline
$\bullet$ & Implemented as a system of periodic/sporadic tasks\\ \hline
$\bullet$ &  Stringent timing requirements\\ \hline
$\bullet$ & Worst-case bounds are known for all loops \\ \hline
$\bullet$ & No dynamically loaded or self modified codes \\ \hline
$\bullet$ & Recursion is either not used or statically bounded \\ \hline
$\bullet$ & Memory and processing power is often limited \\
\hline\end 
{tabular}
\end{table}



% \end{document}
